Scaling Diffusion Policy in Transformer to 1 Billion Parameters for Robotic Manipulation

Diffusion Policy is a powerful technique tool for learning end-to-end visuomotor robot control. It is expected that Diffusion Policy possesses scalability, a key attribute for deep neural networks, typically suggesting that increasing model size would lead to enhanced performance. However, our observations indicate that Diffusion Policy in transformer architecture (\DP) struggles to scale effectively; even minor additions of layers can deteriorate training outcomes. To address this issue, we introduce Scalable Diffusion Transformer Policy for visuomotor learning. Our proposed method, namely \textbf{\methodname}, introduces two modules that improve the training dynamic of Diffusion Policy and allow the network to better handle multimodal action distribution. First, we identify that \DP~suffers from large gradient issues, making the optimization of Diffusion Policy unstable. To resolve this issue, we factorize the feature embedding of observation into multiple affine layers, and integrate it into the transformer blocks. Additionally, our utilize non-causal attention which allows the policy network to \enquote{see} future actions during prediction, helping to reduce compounding errors. We demonstrate that our proposed method successfully scales the Diffusion Policy from 10 million to 1 billion parameters. This new model, named \methodname, can effectively scale up the model size with improved performance and generalization. We benchmark \methodname~across 50 different tasks from MetaWorld and find that our largest \methodname~outperforms \DP~with an average improvement of 21.6\%. Across 7 real-world robot tasks, our ScaleDP demonstrates an average improvement of 36.25\% over DP-T on four single-arm tasks and 75\% on three bimanual tasks. We believe our work paves the way for scaling up models for visuomotor learning. The project page is available at scaling-diffusion-policy.github.io.

==> describe_exp.tex <==
\begin{itemize}
    \item \textbf{Close Laptop.} The robot needs to \ding{172} Move to the back of the laptop and close its gripper. \ding{173} Push the back of the laptop until it is completely closed.
    \item \textbf{Stack Cube.} The robot needs to accurately \ding{172} Capture the position of a randomly placed blue cube and then stacks it on top of the pink cube.
    \item \textbf{Flip Mug.} The robot needs to \ding{172} Pickup a randomly placed mug. \ding{173} Place it lip up.
    \item \textbf{Place Tennis.} The robot needs to \ding{172} Grasp the tennis ball as close to its center of gravity as possible. \ding{173} Place it into the tennis bucket.
    
    \item \textbf{[Bimanual] Stack Cube.} The robot needs to \ding{172} Pick up both cubes. \ding{173} Place the purple cube on the green plate. \ding{174} Place the orange cube on the top of purple cube.
    
    \item \textbf{[Bimanual] Put Tennis Ball into Bag.} The robot needs to \ding{172} Pick the zipper and grasp the right side of the bag. \ding{173} Unzip the bag. \ding{174} Open the bag. \ding{175} Place the tennis ball into the bag.
    
    \item \textbf{[Bimanual] Sweep Trash.} The robot needs to \ding{172} Push the broom by left arm. \ding{173} Grasp the broom by the right arm. \ding{174} Sweep the trash into the dustpan. \ding{175} Place the broom on the top of dustpan.
\end{itemize}

==> unmask_exp.tex <==
\begin{table}[t]
\centering
\caption{Ablation study on the effectiveness of non-causal attention on real-world tasks. The experiments are conducted on bimanual UR5 robot.}
\label{tab:unmask}
\resizebox{0.47\textwidth}{!}{\begin{tabular}{c|c|c|c|c|c}
\toprule
\textbf{Model} & Non-causal & Task1 & Task2 & Task3 & \textbf{Avg.} \\
\midrule
% \midrule
% Octo~\cite{team2024octo}            & \textbf{100} & 70	& 50 & 73.33$\pm$20.54  \\
%\methodname-XS                      & 90 & 80 & 40 & 35 & 61.25$\pm$24.08\\ 
\multirow{2}{*}{\methodname-S} & \xmark                      & 70 & 20 & \textbf{10} &  33.33                                     \\
                               & \cmark                     & \textbf{100} & \textbf{50} & \textbf{10} & \textbf{53.33}_{\textcolor{blue}{+20}}  \\ 
                               \midrule
\multirow{2}{*}{\methodname-B} & \xmark                       & 90 & 50 & \textbf{10} & 50.00 \\
                               & \cmark                     & \textbf{100} & \textbf{60} & \textbf{10} & \textbf{56.67}_{\textcolor{blue}{+6.67}}  \\ 
                               \midrule
\multirow{2}{*}{\methodname-L} & \xmark                       & \textbf{100} & \textbf{80} & 20 & 66.66 \\
                               & \cmark                     & \textbf{100} & \textbf{80} & \textbf{90} & \textbf{90.00}_{\textcolor{blue}{+23.34}} \\ 
\bottomrule
\end{tabular}}
\end{table}

